Ab initio symmetry-adapted approaches to nuclear reactions

In this review, we discuss recent applications of the ab initio symmetry-adapted no-core shell-model (SA-NCSM) theory for study and prediction of structure and reactions of stable and unstable nuclei from light to medium mass range. We explore structure properties of neutron-rich He, Mg, and Li isotopes, with a focus on nuclear collectivity, clustering, and spectroscopic factors, as well as multi-particle excitations of utmost significance in the proximity of the drip lines. In addition, we present extensions of the SA-NCSM with continuum for determining the microscopic structure of reaction fragments, which enables calculations of reaction cross sections for targets from the lightest $^{4,6}$He to $^{40}$Ca, rooted in first principles. We illustrate this for neutron and proton elastic scattering, deuteron and alpha capture reactions, and alpha knock-out reactions. Furthermore, we discuss microscopic optical potentials with uncertainty quantification, a critical ingredient in many reaction models, and reaction observables with uncertainties that stem from the underlying chiral potential. We also discuss the impact of alpha clustering on reactions of significance to nuclear astrophysics, as well as on beta decays and beyond-the-standard-model physics.

==> elsarticle/doc/tmp.tex <==
....
....

\end{abstract}

%%Graphical abstract
\begin{graphicalabstract}
%\includegraphics{grabs}
\end{graphicalabstract}

%%Research highlights
\begin{highlights}
\item Research highlight 1
\item Research highlight 2
\end{highlights}

\begin{keyword}
%% keywords here, in the form: keyword \sep keyword
....
....

